Can Synthetic Translations Improve Bitext Quality?

Synthetic translations have been used for a wide range of NLP tasks primarily as a means of data augmentation. This work explores, instead, how synthetic translations can be used to revise potentially imperfect reference translations in mined bitext. We find that synthetic samples can improve bitext quality without any additional bilingual supervision when they replace the originals based on a semantic equivalence classifier that helps mitigate NMT noise. The improved quality of the revised bitext is confirmed intrinsically via human evaluation and extrinsically through bilingual induction and MT tasks.

==> tables/speedingup.tex <==
\begin{table}[!t]
    \centering
    \scalebox{0.65}{
    \begin{tabular}{lll}
    
    & \multicolumn{1}{c}{\textsc{uni-nmt}} & \multicolumn{1}{c}{\textsc{bi-nmt}}\\
    \rowcolor{gray!10}
    \multicolumn{3}{l}{\textit{\en} \rightarrow \textit{\el}} \\ 
    \addlinespace[0.2em]
     %                       & Uni-T & Bi-T\\\cline{2-3}
    %\textcolor{gray}{\textit{Teacher}}        & \textcolor{gray}{$26.84$} & \textcolor{gray}{$27.32$} \\
    Equivalized bitext     & $27.89\pm0.29$ & $27.92\pm0.06$ \\ 
    + Augmentation  & $28.01\pm0.16$     & $27.89\pm0.24$ \\
    
    \addlinespace[0.3em]
    
    \rowcolor{gray!10}
    \multicolumn{3}{l}{\textit{\el} \rightarrow \textit{\en}} \\ 
    \addlinespace[0.2em]
  
    %                        & \textsc{Uni-T} & \textsc{Bi-T}\\\cline{2-3}
    %\textcolor{gray}{\textit{Teacher}}        & \textcolor{gray}{$28.15$}        & \textcolor{gray}{$28.57$}\\
     Equivalized bitext        & $29.63\pm0.29$ & $29.57\pm0.36$\\ 
    + Augmentation & $29.90\pm0.24$ & $29.68\pm0.14$\\   
    
    \addlinespace[0.3em]

    \rowcolor{gray!10}
    \multicolumn{3}{l}{\textsc{ro} \rightarrow \textit{\en}} \\ 
    \addlinespace[0.2em]
   
    %                         & \textsc{Uni-T} & \textsc{Bi-T}\\\cline{2-3}
    %\textcolor{gray}{\textit{Teacher}}         &  \textcolor{gray}{$23.64$}
    %& \textcolor{gray}{$24.52$}\\
    Equivalized bitext       &  $24.54\pm0.06$        & $24.69\pm0.11$\\ 
    + Augmentation  &  $24.81\pm0.11$        & $24.82\pm0.04$\\  
   
    \addlinespace[0.3em]
 
    \rowcolor{gray!10}
    \multicolumn{3}{l}{\textsc{en} \rightarrow \textsc{ro}} \\ 
    \addlinespace[0.2em]
   
    %                         & \textsc{Uni-T} & \textsc{Bi-T}\\\cline{2-3}
    %\textcolor{gray}{\textit{Teacher}}         & \textcolor{gray}{$20.51$}  &
    %\textcolor{gray}{$20.63$} \\
    Equivalized bitext         & $20.84\pm0.04$         & $20.73\pm0.12$\\ 
    + Augmentation  &   $20.95\pm0.08$        & $20.75\pm0.05$ \\  
    
    \end{tabular}}
    \caption{\bleu scores for \textsc{nmt} on equivalized bitexts using uni- (\textsc{uni-nmt})  vs. bi-directional \nmt models (\textsc{bi-nmt}). Equivalizing the bitext with \textsc{bi-nmt} \textsc{nmt} yields comparable \bleu  with \textsc{uni-nmt}.%, while using single models. 
    %\eb{I excluded the performance of what I was calling ``teachers'' from the Table as it was confusing what it should compare to. I am planning on commenting on their performance on a footnote in the main text.}
    }
    \label{tab:speedng_up}\vspace{-1em}
\end{table}


\subsection{MT evaluation of fine-tuning mT5}

\begin{figure}[!ht]
    \centering
    \includegraphics[scale=0.12]{analysis_figs/mt5.drawio.pdf}
    \caption{mT5 fine-tuned}
    \label{fig:mt5}
\end{figure}

\subsection{Evaluation on Bilingual Lexicon Induction}

\paragraph{Main Results} Table~\ref{tab:BLI_main}

\begin{table}[!ht]
    \centering
    \scalebox{0.85}{
    \begin{tabular}{llllll}
    \rowcolor{gray!10}
     Pair   & Bitext     & All & [1,5) & [5,100) & >100 \\
        \multirow{2}{*}{\rotatebox{0}{\textsc{el-en}}} & Original     & $76.2$ & $59.4$ & $76.6$ & $81.4$\\
                                                        & Equivalized  & $\mathbf{77.6^*}$ &  $\mathbf{60.4^*}$ & $\mathbf{78.4^*}$ & $81.6$\\
        \addlinespace[0.2cm]
                                       
       \multirow{2}{*}{\rotatebox{0}{\textsc{en-ro}}}  & Original     & $89.2$ & $78.6$ & $86.9$ & $87.1$\\
                                                        & Equivalized  & $\mathbf{90.8^*}$ & $\mathbf{80.0^*}$ & $\mathbf{87.5^*}$ & $86.9$\\
    \end{tabular}}
    \caption{Precision results on \textsc{muse} datasets for unsupervised \textsc{bli} tasks. Equivalized bitexts yield statistically significant ($*$) improvements over the original bitexts for low-to-medium frequency dictionary entries.}
    \label{tab:BLI_main}
\end{table}  


\begin{table}[!ht]
    \centering
        \scalebox{0.5}{
    \begin{tabular}{llllll}
        αστεροειδές & star	              & 	?       & απόστολος & apostolos    & \xmark \\ 
        προσφέρεται & offers	          &  \cmark	    & βραχνό & raucous         &  \xmark \\  
        κεραυνός & keravnos	              &  \xmark     & μπανζούλ & bangaon       & \xmark \\ 
        συμπυκνώνει & encapsulates	      & 	?       & βοηθητικές & auxiliary   & \cmark\\
        σεξτέτο & sexteto	              & \cmark 	    & ομιλήτρια & spokesperson & \cmark \\
        επιχειρηματολογία & argumentation & \cmark 	    & πρωτεργάτη & forerunner  &  \xmark \\
        επίπλωση & furniture	          & \cmark  	& αντιτρομοκρατική & anti-terrorist & \cmark \\
        μπουγκ & bug	                  & \xmark 	    & πλεκτά            & sweaters      & \cmark \\ 
        σχετικοί & related	              & \cmark 	    & εμβολιαστεί & vaccinated &    \cmark \\
        δορυφόρους & moons	              & \xmark 	    & αταξινόμητες & unclassified &  \cmark \\
        δειλή & timid	                  & \cmark	    & στέιν & steen                 & \xmark \\ 
        χάντινγκτον & huntingdon	      & \cmark 	    & χιλιοστό & millimeter & \cmark \\
        ποσότητες & amounts	              & \cmark	    & σελεστίν & célestine & \cmark \\
        πλακέ & squamous	              & \cmark 	    & κόβατς & kovács & \xmark\\
        αποποίηση & relinquishing	      & ?       	& σεμίνα & omni & \xmark \\
        ατμούς & vapors	                  & \cmark 	    & σπάιντερμαν & spider-man & \cmark \\
        τερματισμοί & endings	          & \cmark  	& πάνω & over & \cmark \\
        αλεξανδρινό & alexandrine	      & \cmark  	& ενδιαφέρων & love & \xmark \\
        σπασμοί & fits	                  & ? 	        & αγριόγατες & cats &      \xmark \\ 
        σίδερα & sidelines	              & \xmark	    & αγορα & trade & \cmark \\
        συνοδεύονται & are	              & \xmark 	    & επικεφαλίδα & header & \cmark \\ 
        διανέμονται & are	              & \xmark  	& μάσλοου & khan & \xmark \\
        θραύση & fracturing	              & \cmark  	& τεχνητά & artificially & \cmark \\
        κυβερνά & rule	                  & \cmark  	& πέτροβιτς & petrović & \cmark \\
        συνάξεις & meetings	              & \cmark  	& ανθίζει & flowers & \cmark \\
        χριστιανία & christianity	      & \cmark  	& ζήτω & vive & \xmark \\
        απειλούνται  & are	              & \xmark 	    & τυλίγει & picks & \xmark \\
        ποινικοποίηση & penalize	      & \cmark 	    & μπαέζ & ross & \xmark \\
        στερέωμα & stardom	              & \xmark 	    & φιλοδοξεί & is & \xmark \\
        τζαπ & elford	                  & \xmark 	    & τρυφερή & loving & ? \\
        ταυρομαχία & bullfighting	      & \cmark 	    & σωρός & remains & \xmark \\
        χειρός & handbags	              & ? 	        & χαλυβουργεία & works & \xmark \\
        κδ & cd	                          & ? 	        & μάιρα & chloe & \xmark \\
        τρομοκρατεί & terrorizes	      & \cmark 	    & συγκλόνισε & shocked & \cmark \\ 
        μακέι & mackey	                  & \cmark 	    & άτακτη & mischievous & \cmark \\
        ζάκυνθο & zakynthos	              & \cmark 	    & οταν & after & ?  \\
        συμπτωματολογία & symptomology	  & \cmark	    & εντομοφάγα & insectivores & \cmark \\
        πολυφυλετική & polyphyletic	      & \cmark 	    & κραδασμούς & vibrations & \cmark \\
        κούνια & cunha	                  & \xmark 	    & μπελάς & nuisance & \cmark \\
        καταβεβλημένος & overcome	      & \cmark 	    & πάστες & pastries & \cmark \\
        απάτες & scams	                  & \cmark 	    & διασπαστική & divisive & \cmark \\
        γιάννη & giannis	              & \cmark 	    & κατάληψη & capture & \xmark \\
        δηλητηριάσεις & poisonings	 & \cmark	   & παραδίδονται & surrender & \cmark \\
        φιλόξενοι & colorful	     & \xmark 	   & κλήρων & clergy & \cmark \\
        φημισμένος & renowned	     & \cmark      & σκεύη & vessels & \cmark \\
        φουσκωμένα & filled	         & ? 	       & λεπτονίων & leptons & \cmark \\
        υπονοούμενα & undertones	 & \cmark	   & εξάγονται & are & \xmark \\
        όριο & boundary	             & \cmark 	   & απότομο & abrupt & \cmark \\
        χαλάρωσε & relaxed	         & \cmark 	   & παρασυμπαθητικό & sympathetic & ? \\
        αισθητικός & aesthetic	     & \cmark 	   & ταρίχευση & embalming & \cmark \\
        ταμαντούα & tamanduas	     & \cmark 	   & κεκτημένο & precedent & \xmark \\
        εστίες & foci	             & ?	       & καλκούτα & kolkata & \cmark \\
        θεωρείται & is	             & \xmark 	   & σίρι & sirri & \cmark \\
        κορμό & trunk	             & \cmark 	   & ξεπερασμένο & obsolete & \cmark \\
        σπύρο & spyros	             & \cmark 	   & ανώμαλος & bumpy & \cmark \\
        αναισθητικά & anesthetics	 & \cmark	   & εξισορρόπησης & substance & \xmark \\
        στρατηγικές & strategic	     & \cmark 	   & πολυσακχαρίτης & polysaccharides & \cmark \\
        αναπνέει & breathe	         & \cmark 	   & επίπονες & persistent & \cmark \\
        εξουδετερώσει & neutralize	 & \cmark 	   & αμφιθέατρο & amphitheatre & \cmark \\
        μελαγχολική & melancholic	 & 	\cmark     & αναπληρωματικό & an & \xmark \\
        θυμήθηκε & recalled	         & \cmark 	   & εντελώς & entirely & \cmark\\
        πασχαλίτσα & ladybird	     & \cmark 	   & λιθόστρωτο & cobbled & \cmark \\
        πυροκροτητές & caps	         & ? 	       & διοικητικοί & administrative & \cmark \\
        κραυγαλέα & screaming	     & ? 	       & κομιστής & bearer & \cmark \\
        μολδαβίας & moldavia	     & \cmark 	   & συλλογικότητες & competitions & \xmark \\
        σαλιγκάρι & shilling	     & \xmark 	   & χουλιγκανισμού & micromanagement & \xmark \\
        ενισχυθεί & enhance	         & \cmark 	   & τσάρους & tsars & \cmark \\
        πρεσβυτέριο & presbytery	 & \cmark	   & ντόνελ & dorff & \xmark \\
        μάγιστρος & master	         & \cmark 	   & κίραν & kiran & \cmark \\
        αλτ & alt	                 & \cmark 	   & πρωτοποριακή & pioneering & \cmark \\
        χρονολογία & date	         & \cmark 	   & λένοξ & brookline & \xmark \\
        κανένα & any	             & \cmark 	   & λείπουν & are & \xmark \\
        κορμός & road	             & \xmark 	   & εξάντα & astronomy & \xmark \\
        καθαριστήριο & cleanup	     & \xmark 	   & πτωτική & downward & \cmark \\
        ανατεθεί & assigned	         & \cmark 	   & αρχιτεκτονικές & architectural & \cmark \\
        εξοικονόμηση & save	         & \cmark 	   & γαλλόφωνο & french-speaking & \cmark \\
        μπαρακούντα & barracudas	 & \cmark	   & μέντε & mede & \xmark \\
        ταυτοποίησης & identification	 & \cmark	   & εκθρονίζοντας & deposing & \cmark \\ 

    \end{tabular}}
    \caption{Ground-truth analysis on false positives. $65/80$ andf $51/80$ false positives are correct for the equivalized and original bitexts, respectively.}
    \label{tab:ground_truth_bli}
\end{table}

